Recent Advances in DRAM and Flash Memory Architectures

This article features extended summaries and retrospectives of some of the recent research done by our group, SAFARI, on (1) understanding, characterizing, and modeling various critical properties of modern DRAM and NAND flash memory, the dominant memory and storage technologies, respectively; and (2) several new mechanisms we have proposed based on our observations from these analyses, characterization, and modeling, to tackle various key challenges in memory and storage scaling. In order to understand the sources of various bottlenecks of the dominant memory and storage technologies, these works perform rigorous studies of device-level and application-level behavior, using a combination of detailed simulation and experimental characterization of real memory and storage devices.

==> acks.tex <==
\section*{Acknowledgments}

The works featured in this issue, along with our related works that
we reference in each feature, are a
result of the research done together with many students and
collaborators over the course of the past 10+ years, whose
contributions we acknowledge.
In particular, we acknowledge and appreciate the dedicated effort 
of current and former students and postdocs in our research group, 
including
Amirali Boroumand,
Yu Cai,
Kevin Chang,
Chris Fallin,
Juan G{\'o}mez Luna,
Rachael Harding,
Hasan Hassan,
Kevin Hsieh,
Tyler Huberty, 
Ben Jaiyen,
Abhijith Kashyap,
Samira Khan, 
Jeremie Kim, 
Yoongu Kim, 
Tianshi Li, 
Yang Li, 
Jamie Liu, 
Donghyuk Lee, 
Yixin Luo, 
Justin Meza, 
Minesh Patel,
Gennady Pekhimenko, 
Ivan Puddu
Mohammad Sadr,
Vivek Seshadri, 
Ashish Shrestha,
Lavanya Subramanian, 
Arash Tavakkol
Nandita Vijaykumar, 
Abdullah Giray Ya{\u g}l{\i}k{\c c}{\i},
HanBin Yoon, and
Jishen Zhao.

Aside from our featured
works and other referenced papers from our group, where a wealth
of information on modern memory and storage systems can be found, at least eight
Ph.D.\ dissertations have shaped the research directions we have pursued:
\begin{itemize}[leftmargin=1.6em]
\item Yu Cai's thesis
entitled ``NAND Flash Memory: Characterization, Analysis, Modeling and
Mechanisms''~\cite{cai.thesis12}

\item Lavanya Subramanian's thesis entitled ``Providing
High and Controllable Performance in Multicore Systems Through Shared
Resource Management''~\cite{subramanian.thesis15}

\item Yoongu Kim's thesis
entitled ``Architectural Techniques to Enhance DRAM
Scaling''~\cite{kim.thesis15}

\item Donghyuk Lee's thesis entitled
``Reducing DRAM Latency at Low Cost by Exploiting
Heterogeneity''~\cite{lee.thesis16}

\item Vivek Seshadri's
thesis entitled ``Simple DRAM and Virtual Memory Abstractions to
Enable Highly Efficient Memory Subsystems''~\cite{seshadri.thesis16}

\item Gennady Pekhimenko's thesis entitled ``Practical Data Compression for
Modern Memory Hierarchies''~\cite{pekhimenko.thesis16}

\item Kevin Chang's thesis entitled ``Understanding and
Improving the Latency of DRAM-Based Memory
Systems''~\cite{chang.thesis17}

\item Rachata Ausavarungnirun's
thesis entitled ``Techniques for Shared Resource Management in Systems
with Throughput Processors''~\cite{ausavarungnirun.thesis17}.
\end{itemize}

We also acknowledge various funding agencies (the National Science
Foundation, the Semiconductor Research Corporation, the Intel Science and
Technology Center on Cloud Computing, CyLab, the CMU Data Storage
Systems Center, and the NIH) and
industrial partners (AMD, Facebook, Google, HP Labs, Huawei, IBM,
Intel, Microsoft, NVIDIA, Oracle, Qualcomm, Rambus, Samsung, Seagate,
VMware), and ETH Z{\"u}rich, who have supported the featured works in
this issue and other related work generously over the years.
